ORCA: A Network and Architecture Co-design for Offloading us-scale Datacenter Applications

Responding to the "datacenter tax" and "killer microseconds" problems for datacenter applications, diverse solutions including Smart NIC-based ones have been proposed. Nonetheless, they often suffer from high overhead of communications over network and/or PCIe links. To tackle the limitations of the current solutions, this paper proposes ORCA, a holistic network and architecture co-design solution that leverages current RDMA and emerging cache-coherent off-chip interconnect technologies. Specifically, ORCA consists of four hardware and software components: (1) unified abstraction of inter- and intra-machine communications managed by one-sided RDMA write and cache-coherent memory write; (2) efficient notification of requests to accelerators assisted by cache coherence; (3) cache-coherent accelerator architecture directly processing requests received by NIC; and (4) adaptive device-to-host data transfer for modern server memory systems consisting of both DRAM and NVM exploiting state-of-the-art features in CPUs and PCIe. We prototype ORCA with a commercial system and evaluate three popular datacenter applications: in-memory key-value store, chain replication-based distributed transaction system, and deep learning recommendation model inference. The evaluation shows that ORCA provides 30.1~69.1% lower latency, up to 2.5x higher throughput, and 3x higher power efficiency than the current state-of-the-art solutions.

==> ack.tex <==
% !TEX root = paper.tex
\section*{Acknowledgment}
\label{sec:ack}
We would like to thank xxx as well as the anonymous reviewers for their insightful and helpful information and feedback. 
We also thank Zeran Zhu, Jiacheng Ma, Nikita Lazarev, Shaojie Xiang for their technical support and discussion. 
This research is supported by National Science Foundation (No. CNS-1705047), Intel Corporation’s Academic research funding, and NVIDIA device donation.
